Does Audio Deepfake Detection Generalize?

Current text-to-speech algorithms produce realistic fakes of human voices, making deepfake detection a much-needed area of research. While researchers have presented various techniques for detecting audio spoofs, it is often unclear exactly why these architectures are successful: Preprocessing steps, hyperparameter settings, and the degree of fine-tuning are not consistent across related work. Which factors contribute to success, and which are accidental? In this work, we address this problem: We systematize audio spoofing detection by re-implementing and uniformly evaluating architectures from related work. We identify overarching features for successful audio deepfake detection, such as using cqtspec or logspec features instead of melspec features, which improves performance by 37% EER on average, all other factors constant. Additionally, we evaluate generalization capabilities: We collect and publish a new dataset consisting of 37.9 hours of found audio recordings of celebrities and politicians, of which 17.2 hours are deepfakes. We find that related work performs poorly on such real-world data (performance degradation of up to one thousand percent). This may suggest that the community has tailored its solutions too closely to the prevailing ASVSpoof benchmark and that deepfakes are much harder to detect outside the lab than previously thought.

==> img/table.tex <==
\begin{tabular}{lrr}
\toprule
{} &     len\_spoof &    len\_benign \\
speaker                         &               &               \\
\midrule
2Pac                            &    479.137914 &    285.387982 \\
Adam Driver                     &    712.406077 &    497.005125 \\
Alan Watts                      &    998.327846 &    303.057052 \\
Alec Guinness                   &  10019.115510 &   5719.856599 \\
Alexandria Ocasio-Cortez        &    876.393968 &   1354.311791 \\
Arnold Schwarzenegger           &    410.026893 &    895.772925 \\
Ayn Rand                        &   5469.525941 &   5097.460771 \\
Barack Obama                    &   1329.066984 &  13285.828073 \\
Bernie Sanders                  &   6926.089615 &   6476.370159 \\
Bill Burr                       &    517.257914 &    853.048435 \\
Bill Clinton                    &   3035.282857 &   3194.235238 \\
Billie Eilish                   &     66.868934 &     71.995011 \\
Bob Ross                        &    308.839773 &    326.070023 \\
Boris Johnson                   &    565.659864 &    851.932018 \\
Calvin Coolidge                 &    131.970975 &    219.613923 \\
Christopher Hitchens            &   2817.756009 &   3119.775465 \\
Dave Chappelle                  &     77.229977 &     87.491020 \\
Donald Trump                    &    828.964036 &  11723.674422 \\
Dwight Eisenhower               &    287.390975 &    619.311655 \\
FDR                             &   1083.514921 &   1030.104218 \\
Frank Sinatra                   &    310.762041 &     90.259002 \\
George Carlin                   &    574.060952 &    845.649796 \\
George W. Bush                  &    595.820045 &    235.684127 \\
Gilbert Gottfried               &    955.229841 &    476.683991 \\
Harry Truman                    &    100.472971 &    228.153923 \\
Homer Simpson                   &     25.783991 &     11.000000 \\
JFK                             &   1179.637868 &   1150.031383 \\
Jeff Goldblum                   &     30.034966 &    308.274966 \\
Jerry Seinfeld                  &    312.445896 &     65.904989 \\
Jimmy Carter                    &     98.226984 &     63.666122 \\
Joe Rogan                       &    111.356054 &     35.952018 \\
John Cleese                     &    864.011882 &    433.429841 \\
Kamala Harris                   &     25.832971 &    126.203991 \\
Kanye West                      &    503.871882 &    313.623855 \\
Louis C.K.                      &    435.487891 &     66.278957 \\
Louis Farrakhan                 &    706.348889 &   1036.494150 \\
Lyndon Johnson                  &    108.116961 &    299.118549 \\
Malcolm X                       &    227.744989 &    597.983991 \\
Mark Zuckerberg                 &   1480.449932 &   2068.501270 \\
Martin Luther King              &   1558.893651 &   1671.674694 \\
Milton Friedman                 &   1474.819819 &   1276.040091 \\
Mitch Hedberg                   &    201.383946 &     33.000000 \\
Mr. Rogers                      &    552.491927 &    140.874830 \\
Nelson Mandela                  &    930.860000 &    278.072018 \\
Nick Offerman                   &     80.746984 &    572.270068 \\
Norm MacDonald                  &    588.013016 &    207.637914 \\
Orson Welles                    &   1121.601995 &    105.639093 \\
Queen Elizabeth II              &   1486.318685 &    627.532018 \\
Richard Nixon                   &    541.616054 &    749.812063 \\
Robert Kardashian               &     78.565034 &    350.774830 \\
Ronald Reagan                   &   4423.346032 &   2063.536463 \\
Scarlett Johansson              &    327.185941 &    200.284943 \\
Sergeant Hartman (R. Lee Ermey) &     97.168980 &     46.000000 \\
The Notorious B.I.G.            &   1046.252880 &     67.291020 \\
Tom Lehrer                      &    105.330975 &     24.000000 \\
Tucker Carlson                  &    443.321950 &    216.632971 \\
William F. Buckley              &     93.512018 &     35.421995 \\
Winston Churchill               &   1141.827982 &   1706.180227 \\
\bottomrule
\end{tabular}


==> tables/old/best-asvspoof.tex <==
\begin{tabular}{lrrr}
\toprule
           &  eer\_test\_unknown &  eer\_YT &     t-dcf \\
 Feature Type &                   &                      &           \\
\midrule
  cqtspec &          0.147979 &             0.597144 &  0.322596 \\
       logspec &          0.136377 &             0.721902 &  0.307750 \\
       melspec &          0.234867 &             0.698612 &  0.448054 \\
       raw &          0.124166 &             0.366310 &  0.239657 \\
\bottomrule
\end{tabular}


==> tables/old/best-youtube.tex <==
\begin{tabular}{lrrr}
\toprule
           &  eer\_test\_unknown &  eer\_YT &     t-dcf \\
 Feature Type &                   &                      &           \\
\midrule
  cqtspec &          0.147979 &             0.597144 &  0.322596 \\
       logspec &          0.136377 &             0.721902 &  0.307750 \\
       melspec &          0.234867 &             0.698612 &  0.448054 \\
       raw &          0.124166 &             0.366310 &  0.239657 \\
\bottomrule
\end{tabular}


==> tables/old/feat_subsel.tex <==
\begin{tabular}{lrrr}
\toprule
{} &  eer\_test\_unknown &  eer\_test\_unknown\_YT &     t-dcf \\
Feat. Subsel. &                   &                      &           \\
\midrule
-1            &          0.202194 &             0.600249 &  0.379573 \\
 4            &          0.207094 &             0.664638 &  0.405438 \\
\bottomrule
\end{tabular}


==> tables/old/feature_no_trim.tex <==
\begin{tabular}{lrrr}
\toprule
     &  \multicolumn{2}{c}{ASVspoof19 eval} &     In-the-Wild Data \\
Feature Type & EER \%       & t-DCF      &  EER \%  \\
\midrule
 cqtspec &         14.306377 &  0.321282 &            64.132301 \\
 logspec &         12.920236 &  0.271511 &            72.433981 \\
 melspec &         19.822462 &  0.409534 &            68.380601 \\
 raw &         11.760109 &  0.229392 &            40.331046 \\
\bottomrule
\end{tabular}



==> tables/old/feature_type.tex <==
\begin{tabular}{lrrr}
\toprule
{} &  eer\_test\_unknown &  eer\_test\_unknown\_YT &     t-dcf \\
Feature Type &                   &                      &           \\
\midrule
cqtspec      &          0.168544 &             0.616128 &  0.361405 \\
logspec      &          0.175520 &             0.767869 &  0.360305 \\
melspec      &          0.294194 &             0.688425 &  0.515237 \\
raw          &          0.190542 &             0.383801 &  0.334043 \\
\bottomrule
\end{tabular}


==> tables/old/original-values.tex <==
\begin{table}
\begin{tabular}{|l|r|r|r|l|l|l|l|}
\hline
Model & Source & input length & source feature &  Src. EER \% & Our EER \% & Src. t-DCF & Our t-DCF \\
\hline \hline
      \crnn/ & \cite{chintha2020Recurrent} & variable & raw & 4.02 & 16.2 & 0.1340 & 0.33 \\
      \drn/ & \cite{alzantot2019Deep} & fixed & mfcc$^\dagger$ & 9.33 & 14.3 & 0.2042 & 0.33\\
      %\meso/ & \cite{afchar2018MesoNet} & & &  & & & \\
      %\mi/ & \cite{afchar2018MesoNet} & & &  & & & \\
      \lcnn/ & \cite{wang2021Comparative} & fixed & lfcc$^\dagger$ & 2.31 & 25.606 & 0.056 & 0.511 \\
      \lcnna/ & \cite{wang2021Comparative} & variable & lfb$^\dagger$ & 3.34 & 6.891 & 0.064 & 0.191\\
      \lcnnl/ & \cite{wang2021Comparative} & variable & lfcc$^\dagger$ & 1.92 & 6.033 & 0.052 & 0.104 \\
      \rn/ & \cite{tak2021EndtoEnd} & fixed & raw & 5.13 & 4.26 & 0.1175 & 0.129 \\
\hline
\end{tabular}
\caption{Comparing results on the ASVspoof 2019 eval set as reported in the sources with our results taken from Table~\ref{tab:results}.
If the source includes one of the features we use (cqtspec, logspec, melspec), we report the one with the highest t-DCF.
If none of the reported results in the source are one of our features, we report the highest result in the source and compare to the highest feature from our own evaluation.
In the latter case we mark the feature with $\dagger$.
We omit \meso/ and \mi/ as they were not evaluated on ASVspoof 2019 data in the source.
The column \emph{input length} indicates whether the source uses variable-length inputs or uses some way of limiting samples to some fixed length.
Our values that are added for comparison reproduce this aspect. However, in favor of using the same length limit and type of padding used in the reference we instead opted to handle all data uniformly across all models.}
\label{tab:source-comparison}
\end{table}

==> tables/old/res.tex <==
\begin{tabular}{llrllll}
\toprule
         Model Name & Feature Type &  Feat. Subsel. &  Trim Sil. Train & eer\_test\_unknown &      t-dcf & eer\_test\_unknown\_YT \\
\midrule
         crnn\_spoof &          raw &             -1 &            False &      15.658±0.35 & 0.312±0.01 &         44.500±8.13 \\
         crnn\_spoof &          raw &             -1 &             True &      39.211±5.98 & 0.537±0.06 &         33.586±0.55 \\
         crnn\_spoof &          raw &              4 &            False &      19.640±1.62 & 0.360±0.04 &         41.710±4.86 \\
         crnn\_spoof &          raw &              4 &             True &      25.519±8.75 & 0.387±0.02 &         40.786±0.06 \\
          lcnn\_wang &      cqtspec &             -1 &            False &       6.354±0.39 & 0.174±0.03 &        65.559±11.14 \\
          lcnn\_wang &      cqtspec &             -1 &             True &      25.107±3.33 & 0.457±0.03 &         79.455±1.36 \\
          lcnn\_wang &      cqtspec &              4 &            False &      25.534±0.10 & 0.512±0.00 &         70.015±4.74 \\
          lcnn\_wang &      cqtspec &              4 &             True &      25.735±1.08 & 0.479±0.01 &         80.616±0.74 \\
          lcnn\_wang &      logspec &             -1 &            False &       7.537±0.42 & 0.141±0.02 &         72.515±2.15 \\
          lcnn\_wang &      logspec &             -1 &             True &      26.496±4.22 & 0.384±0.06 &         87.509±3.41 \\
          lcnn\_wang &      logspec &              4 &            False &      22.271±2.36 & 0.377±0.01 &         91.110±2.17 \\
          lcnn\_wang &      logspec &              4 &             True &      22.337±1.66 & 0.432±0.07 &         89.726±0.54 \\
          lcnn\_wang &      melspec &             -1 &            False &      15.093±2.73 & 0.428±0.05 &         70.311±2.15 \\
          lcnn\_wang &      melspec &             -1 &             True &      34.680±2.90 & 0.558±0.00 &         72.700±0.02 \\
          lcnn\_wang &      melspec &              4 &            False &      30.258±3.38 & 0.503±0.04 &         81.942±3.50 \\
          lcnn\_wang &      melspec &              4 &             True &      26.952±1.49 & 0.468±0.01 &         79.632±2.34 \\
lcnn\_wang\_attention &      cqtspec &             -1 &            False &       6.762±0.27 & 0.178±0.01 &         66.684±1.08 \\
lcnn\_wang\_attention &      cqtspec &             -1 &             True &      32.919±1.48 & 0.507±0.00 &         82.392±3.59 \\
lcnn\_wang\_attention &      cqtspec &              4 &            False &      23.228±3.98 & 0.468±0.06 &         75.317±8.25 \\
lcnn\_wang\_attention &      cqtspec &              4 &             True &      22.769±0.64 & 0.479±0.00 &         82.506±2.61 \\
lcnn\_wang\_attention &      logspec &             -1 &            False &       7.888±0.57 & 0.180±0.05 &         77.122±4.91 \\
lcnn\_wang\_attention &      logspec &             -1 &             True &      24.018±1.10 & 0.439±0.11 &        83.104±13.40 \\
lcnn\_wang\_attention &      logspec &              4 &            False &      14.958±2.37 & 0.354±0.03 &         80.651±6.14 \\
lcnn\_wang\_attention &      logspec &              4 &             True &      19.099±2.27 & 0.450±0.08 &         84.009±5.09 \\
lcnn\_wang\_attention &      melspec &             -1 &            False &      13.487±5.59 & 0.374±0.14 &         70.986±9.73 \\
lcnn\_wang\_attention &      melspec &             -1 &             True &      38.314±0.11 & 0.577±0.01 &         82.809±0.44 \\
lcnn\_wang\_attention &      melspec &              4 &            False &      19.534±2.57 & 0.449±0.02 &         85.118±1.01 \\
lcnn\_wang\_attention &      melspec &              4 &             True &      21.473±2.38 & 0.470±0.02 &         83.137±5.99 \\
     lcnn\_wang\_lstm &      cqtspec &             -1 &            False &       6.228±0.50 & 0.113±0.01 &         71.500±1.37 \\
     lcnn\_wang\_lstm &      cqtspec &             -1 &             True &      28.971±3.24 & 0.518±0.01 &         71.595±1.84 \\
     lcnn\_wang\_lstm &      cqtspec &              4 &            False &      20.857±0.14 & 0.478±0.01 &         72.251±2.97 \\
     lcnn\_wang\_lstm &      cqtspec &              4 &             True &      34.354±6.28 & 0.586±0.10 &        66.258±15.09 \\
     lcnn\_wang\_lstm &      logspec &             -1 &            False &       9.936±1.74 & 0.158±0.01 &         79.109±0.84 \\
     lcnn\_wang\_lstm &      logspec &             -1 &             True &      25.185±9.97 & 0.494±0.04 &         65.299±3.64 \\
     lcnn\_wang\_lstm &      logspec &              4 &            False &      13.018±3.08 & 0.330±0.05 &        79.706±15.80 \\
     lcnn\_wang\_lstm &      logspec &              4 &             True &      17.718±1.38 & 0.452±0.03 &         87.792±3.14 \\
     lcnn\_wang\_lstm &      melspec &             -1 &            False &       9.260±1.33 & 0.240±0.04 &         62.304±0.17 \\
     lcnn\_wang\_lstm &      melspec &             -1 &             True &      36.025±2.07 & 0.572±0.03 &         70.946±0.65 \\
     lcnn\_wang\_lstm &      melspec &              4 &            False &      27.948±4.64 & 0.483±0.03 &         82.857±3.49 \\
     lcnn\_wang\_lstm &      melspec &              4 &             True &      23.224±0.51 & 0.449±0.02 &         76.659±5.23 \\
               lstm &      cqtspec &             -1 &            False &       7.162±0.27 & 0.127±0.00 &        53.711±11.68 \\
               lstm &      cqtspec &             -1 &             True &      14.421±3.88 & 0.358±0.06 &         54.364±3.99 \\
               lstm &      cqtspec &              4 &            False &      14.409±2.19 & 0.382±0.05 &         55.880±0.88 \\
               lstm &      cqtspec &              4 &             True &      23.808±6.83 & 0.517±0.11 &         59.504±5.02 \\
               lstm &      logspec &             -1 &            False &      10.314±0.81 & 0.160±0.00 &         73.111±2.52 \\
               lstm &      logspec &             -1 &             True &      35.813±5.66 & 0.589±0.07 &         63.431±0.62 \\
               lstm &      logspec &              4 &            False &      23.232±0.32 & 0.512±0.00 &         78.071±0.49 \\
               lstm &      logspec &              4 &             True &      21.431±0.47 & 0.491±0.00 &         79.202±0.08 \\
               lstm &      melspec &             -1 &            False &      16.216±2.92 & 0.358±0.00 &         65.957±7.70 \\
               lstm &      melspec &             -1 &             True &      45.628±0.25 & 0.663±0.03 &         69.420±6.33 \\
               lstm &      melspec &              4 &            False &      37.463±0.46 & 0.553±0.01 &         64.297±2.23 \\
               lstm &      melspec &              4 &             True &      39.373±1.27 & 0.575±0.01 &        65.929±11.23 \\
     meso\_inception &      cqtspec &             -1 &            False &      11.353±1.00 & 0.326±0.03 &        50.007±14.69 \\
     meso\_inception &      cqtspec &             -1 &             True &      31.809±1.45 & 0.597±0.06 &        71.390±14.17 \\
     meso\_inception &      cqtspec &              4 &            False &      21.973±4.96 & 0.453±0.09 &        68.192±12.47 \\
     meso\_inception &      cqtspec &              4 &             True &      33.220±1.03 & 0.634±0.00 &        61.014±14.46 \\
     meso\_inception &      logspec &             -1 &            False &      10.019±0.18 & 0.238±0.02 &         37.414±9.16 \\
     meso\_inception &      logspec &             -1 &             True &      19.614±5.65 & 0.445±0.07 &         73.975±4.93 \\
     meso\_inception &      logspec &              4 &            False &      16.377±3.72 & 0.375±0.09 &         72.753±6.62 \\
     meso\_inception &      logspec &              4 &             True &      18.411±1.39 & 0.402±0.04 &         84.622±2.95 \\
     meso\_inception &      melspec &             -1 &            False &      14.058±5.67 & 0.331±0.11 &        61.996±12.65 \\
     meso\_inception &      melspec &             -1 &             True &      38.773±5.37 & 0.630±0.09 &         77.788±0.41 \\
     meso\_inception &      melspec &              4 &            False &      21.484±3.51 & 0.408±0.03 &        51.980±15.32 \\
     meso\_inception &      melspec &              4 &             True &      22.752±1.14 & 0.461±0.01 &         75.671±6.15 \\
           meso\_net &      cqtspec &             -1 &            False &       7.422±1.61 & 0.219±0.07 &        54.544±11.50 \\
           meso\_net &      cqtspec &             -1 &             True &      27.041±9.76 & 0.448±0.13 &         75.472±3.79 \\
           meso\_net &      cqtspec &              4 &            False &      20.395±2.03 & 0.426±0.06 &         65.928±2.57 \\
           meso\_net &      cqtspec &              4 &             True &      26.731±2.08 & 0.476±0.03 &         71.463±4.62 \\
           meso\_net &      logspec &             -1 &            False &       8.369±1.06 & 0.170±0.05 &         46.939±5.81 \\
           meso\_net &      logspec &             -1 &             True &      19.684±1.95 & 0.383±0.06 &        55.333±16.36 \\
           meso\_net &      logspec &              4 &            False &      11.124±0.79 & 0.263±0.03 &        80.707±12.03 \\
           meso\_net &      logspec &              4 &             True &      13.893±1.63 & 0.341±0.02 &        76.256±15.07 \\
           meso\_net &      melspec &             -1 &            False &      11.305±1.80 & 0.321±0.06 &        58.405±11.28 \\
           meso\_net &      melspec &             -1 &             True &      39.011±1.11 & 0.610±0.04 &         76.669±4.67 \\
           meso\_net &      melspec &              4 &            False &      21.761±0.26 & 0.467±0.00 &        64.415±15.68 \\
           meso\_net &      melspec &              4 &             True &      21.795±3.96 & 0.452±0.06 &         75.558±0.65 \\
            rawnet2 &          raw &             -1 &            False &       7.392±0.46 & 0.114±0.01 &         41.172±3.61 \\
            rawnet2 &          raw &             -1 &             True &      32.541±2.84 & 0.494±0.01 &         58.783±2.21 \\
            rawnet2 &          raw &              4 &            False &       4.351±0.29 & 0.132±0.01 &         33.943±2.59 \\
            rawnet2 &          raw &              4 &             True &      17.463±4.77 & 0.357±0.04 &         44.267±2.04 \\
\bottomrule
\end{tabular}


==> tables/old/table-related-work.tex <==
% Whitespace between columns was a little bit small IMO, so I increased it a bit
\setlength{\tabcolsep}{4pt}
\begin{table}
    \begin{tabular}{l p{0.35\linewidth} p{0.35\linewidth} l}
        \hline
        \hline
        Name & Architecture & Input sample length & Ref. \\
        \hline
        \hline
        ResNet & CNN + Residual blocks & flexible (max) & \cite{alzantot2019Deep} \\
        \hline
        CNN & CNN & last / first 4 seconds of data & \cite{chettri2019Ensemble} \\
        CRNN & CRNN & truncated or looped to first 5 seconds & \cite{chettri2019Ensemble}\\
        1D-CNN & 1D-CNN & looped or random sub-sample of 3.7 seconds & \cite{chettri2019Ensemble} \\
        Wave U-Net & Wave U-Net & pad with silence to 12.23 seconds & \cite{chettri2019Ensemble} \\
        \hline
        CRNNSpoof & CNN + LSTM, inspired by Xception-Net & flexible (RNN) & \cite{chintha2020Recurrent} \\
        WIRENetSpoof & Wide blocks with multiple paths & trimmed or repeated to 4 seconds & \cite{chintha2020Recurrent} \\
        \hline
        GRCNN & GRCNN + CNN that learn signal-to-noise-mask & flexible (RNN) & \cite{gomez-alanis2019Gated} \\
        \hline
        LCNNRaw & LCNN & trimmed or padded with zero & \cite{wang2021Comparative} \\
        LCNNAttention & LCNN + Attention & flexible & \cite{wang2021Comparative} \\
        LCNNLSTM & LCNN + LSTM & flexible (RNN) & \cite{wang2021Comparative} \\
        \hline
        DenseNet & Densely connected CNN & flexible (mean) & \cite{wang2020Densely} \\
        \hline
        \hline
    \end{tabular}
    \caption{Caption}
    \label{tab:original}
\end{table}

==> tables/old/trim.tex <==
\begin{tabular}{llrrrr}
\toprule
                    &              &      &  \multicolumn{2}{c}{ASVspoof19 eval}  & Youtube \\
         Model Name & Feature Type & Clip  &   EER\% &     t-DCF & EER\% \\
\midrule
          \lcnn/ &      cqtspec &             No &         25.107±3.33 & 0.457±0.03 &         79.455±1.36 \\
          \lcnn/ &      cqtspec &              4s &         25.735±1.08 & 0.479±0.01 &         80.616±0.74 \\
          \lcnn/ &      logspec &             No &         26.496±4.22 & \textbf{0.384±0.06} &         87.509±3.41 \\
          \lcnn/ &      logspec &              4s &         \textbf{22.337±1.66} & 0.432±0.07 &         89.726±0.54 \\
          \lcnn/ &      melspec &             No &         34.680±2.90 & 0.558±0.00 &         \textbf{72.700±0.02} \\
          \lcnn/ &      melspec &              4s &         26.952±1.49 & 0.468±0.01 &         79.632±2.34 \\
          \midrule
\lcnna/ &      cqtspec &             No &         32.919±1.48 & 0.507±0.00 &         \textbf{82.392±3.59} \\
\lcnna/ &      cqtspec &              4s &         22.769±0.64 & 0.479±0.00 &         82.506±2.61 \\
\lcnna/ &      logspec &             No &         24.018±1.10 & \textbf{0.439±0.11} &        83.104±13.40 \\
\lcnna/ &      logspec &              4s &         \textbf{19.099±2.27} & 0.450±0.08 &         84.009±5.09 \\
\lcnna/ &      melspec &             No &         38.314±0.11 & 0.577±0.01 &         82.809±0.44 \\
\lcnna/ &      melspec &              4s &         21.473±2.38 & 0.470±0.02 &         83.137±5.99 \\
\midrule
     \lcnnl/ &      cqtspec &             No &         28.971±3.24 & 0.518±0.01 &         71.595±1.84 \\
     \lcnnl/ &      cqtspec &              4s &         34.354±6.28 & 0.586±0.10 &        66.258±15.09 \\
     \lcnnl/ &      logspec &             No &         25.185±9.97 & 0.494±0.04 &         \textbf{65.299±3.64} \\
     \lcnnl/ &      logspec &              4s &         \textbf{17.718±1.38} & 0.452±0.03 &         87.792±3.14 \\
     \lcnnl/ &      melspec &             No &         36.025±2.07 & 0.572±0.03 &         70.946±0.65 \\
     \lcnnl/ &      melspec &              4s &         23.224±0.51 & \textbf{0.449±0.02} &         76.659±5.23 \\
     \midrule
               \lstm/ &      cqtspec &             No &         \textbf{14.421±3.88} & \textbf{0.358±0.06} &         \textbf{54.364±3.99} \\
               \lstm/ &      cqtspec &              4s &         23.808±6.83 & 0.517±0.11 &         59.504±5.02 \\
               \lstm/ &      logspec &             No &         35.813±5.66 & 0.589±0.07 &         63.431±0.62 \\
               \lstm/ &      logspec &              4s &         21.431±0.47 & 0.491±0.00 &         79.202±0.08 \\
               \lstm/ &      melspec &             No &         45.628±0.25 & 0.663±0.03 &         69.420±6.33 \\
               \lstm/ &      melspec &              4s &         39.373±1.27 & 0.575±0.01 &        65.929±11.23 \\
               \midrule
     \mi/ &      cqtspec &             No &         31.809±1.45 & 0.597±0.06 &        71.390±14.17 \\
     \mi/ &      cqtspec &              4s &         33.220±1.03 & 0.634±0.00 &        \textbf{61.014±14.46} \\
     \mi/ &      logspec &             No &         19.614±5.65 & 0.445±0.07 &         73.975±4.93 \\
     \mi/ &      logspec &              4s &         \textbf{18.411±1.39} & \textbf{0.402±0.04} &         84.622±2.95 \\
     \mi/ &      melspec &             No &         38.773±5.37 & 0.630±0.09 &         77.788±0.41 \\
     \mi/ &      melspec &              4s &         22.752±1.14 & 0.461±0.01 &         75.671±6.15 \\
     \midrule
           \meso/ &      cqtspec &             No &         27.041±9.76 & 0.448±0.13 &         75.472±3.79 \\
           \meso/ &      cqtspec &              4s &         26.731±2.08 & 0.476±0.03 &         71.463±4.62 \\
           \meso/ &      logspec &             No &         19.684±1.95 & 0.383±0.06 &        \textbf{55.333±16.36} \\
           \meso/ &      logspec &              4s &         \textbf{13.893±1.63} & \textbf{0.341±0.02} &        76.256±15.07 \\
           \meso/ &      melspec &             No &         39.011±1.11 & 0.610±0.04 &         76.669±4.67 \\
           \meso/ &      melspec &              4s &         21.795±3.96 & 0.452±0.06 &         75.558±0.65 \\
           \midrule
         \crnn/ &          raw &             No &         39.211±5.98 & 0.537±0.06 &         \textbf{33.586±0.55} \\
         \crnn/ &          raw &              4s &         \textbf{25.519±8.75} & \textbf{0.387±0.02} &         40.786±0.06 \\
         \midrule
            \rn/ &          raw &             No &         32.541±2.84 & 0.494±0.01 &         58.783±2.21 \\
            \rn/ &          raw &              4s &         \textbf{17.463±4.77} & \textbf{0.357±0.04} &         \textbf{44.267±2.04} \\
\bottomrule
\end{tabular}


==> tables/old/trim_sil_train.tex <==
\begin{tabular}{lrrr}
\toprule
  &  \multicolumn{2}{c}{ASVspoof19 eval} &     In-the-Wild Data \\
Trim Silence & EER\%       & t-DCF      &  EER\%  \\
\midrule
False           &         15.29 &  0.324 &            65.52 \\
True            &         27.33 &  0.490 &            71.77 \\

\bottomrule
\end{tabular}


==> tables/old/trim_yes_feature_type.tex <==
\begin{tabular}{lrrr}
\toprule
     &  \multicolumn{2}{c}{ASVspoof19 eval} &     In-the-Wild Data \\
Feature Type & EER \%       & t-DCF      &  EER \%  \\
\midrule
cqtspec &         27.240207 &  0.504617 &            71.335825 \\
logspec &         21.974957 &  0.441781 &            77.521582 \\
melspec &         32.333188 &  0.540438 &            75.576526 \\
raw &         28.683455 &  0.443621 &            44.355443 \\
\bottomrule
\end{tabular}

